Less is More: Building Selective Anomaly Ensembles

Ensemble techniques for classification and clustering have long proven effective, yet anomaly ensembles have been barely studied. In this work, we tap into this gap and propose a new ensemble approach for anomaly mining, with application to event detection in temporal graphs. Our method aims to combine results from heterogeneous detectors with varying outputs, and leverage the evidence from multiple sources to yield better performance. However, trusting all the results may deteriorate the overall ensemble accuracy, as some detectors may fall short and provide inaccurate results depending on the nature of the data in hand. This suggests that being selective in which results to combine is vital in building effective ensembles---hence "less is more". In this paper we propose SELECT; an ensemble approach for anomaly mining that employs novel techniques to automatically and systematically select the results to assemble in a fully unsupervised fashion. We apply our method to event detection in temporal graphs, where SELECT successfully utilizes five base detectors and seven consensus methods under a unified ensemble framework. We provide extensive quantitative evaluation of our approach on five real-world datasets (four with ground truth), including Enron email communications, New York Times news corpus, and World Cup 2014 Twitter news feed. Thanks to its selection mechanism, SELECT yields superior performance compared to individual detectors alone, the full ensemble (naively combining all results), and an existing diversity-based ensemble.

==> 050related.tex <==

%\reminder{Shebuti, please reorder lists by number}
We devote this section to related work on ensemble learning, which is the main focus of our work.
For related work on event detection in temporal data, we refer to  \cite{DBLP:journals/corr/AkogluTK14,DBLP:journals/csur/ChandolaBK09,DBLP:journals/tkde/GuptaGAH14}.

%Event detection in temporal data 
%is a fundamental research problem that finds numerous applications in the real world. As such, a large body of research has focused on building effective techniques for this problem. For information on such techniques we refer the reader to detailed surveys \cite{DBLP:journals/corr/AkogluTK14,DBLP:journals/csur/ChandolaBK09,DBLP:journals/tkde/GuptaGAH14} and devote this section to discuss related work on ensemble learning, which is the main focus of our work.


Ensemble techniques leverage multiple different methods to obtain better performance than the individual methods in the ensemble \cite{journals/air/Rokach10}. This is achieved by combining the strengths of accurate methods and alleviating the weaknesses of the less accurate ones. For example, boosting \cite{schapireml90} and stacking \cite{wolpert92} directly integrate accuracy estimation within their iterative ensemble learning. Others assign expertise weights proportional to the accuracy of independent learners and externally combine their results  \cite{HOET1999,juditsky2008,conf/ijcnn/MonteithCSM11,tsybakov04aggregation}.
Ensembles are also known to produce more robust results. For example, 
bootstrap aggregating (or bagging) tends to reduce problems related to over-fitting to the training data \cite{brei96}.

Thanks to these advantages,
% of ensemble learning, a large body of work has been devoted to the study of classification and clustering ensembles
ensemble learning has spurned a large body of work devoted to the study of ensemble classification and clustering \cite{conf/mcs/Dietterich00,conf/icml/FernB03a,conf/sdm/FernL08,books/crc/aggarwal13/GhoshA13,journals/inffus/HadjitodorovKT06,journals/pami/HansenS90,preisach2007,journals/pami/TopchyJP05,conf/wirn/ValentiniM02,journals/tkde/VermaR12,journals/ngc/ZamanH11}. On the other hand, building effective ensembles for anomaly detection has remained to be a challenging task, due to lack of ground truth and inherent objective functions \cite{journals/sigkdd/Aggarwal12,Zimek13Ensemble}.
%As pointed out in recent position articles \cite{journals/sigkdd/Aggarwal12,Zimek13Ensemble},
%one challenge 
%is the lack of ground-truth; which makes it hard to measure detector accuracy apriori and to effectively select accurate detectors to combine, unlike in classification. Moreover, there are no objective or fitness functions for anomaly mining, unlike in clustering.
As such, there exist only a handful of mostly recent works on building anomaly ensembles \cite{conf/pakdd/GaoHZW12,conf/icdm/GaoT06,conf/sdm/KriegelKSZ11,conf/kdd/LazarevicK05,RayanaAkoglu14,conf/sdm/SchubertWZK12,conf/dasfaa/VuAG10,conf/kdd/ZimekGCS13}.
 %\footnote{To the best of our knowledge, this is a comprehensive list.}. 

\hide{ 
conf/kdd/LazarevicK05: the first work on ensembles, same algorithm on different subspaces, combine with max and bfs
conf/icdm/GaoT06, conf/sdm/KriegelKSZ11: unify scores to combine heterogeneous detectors -- full
conf/dasfaa/VuAG10: heterogeneous detectors, how do they combine?--full?
conf/pakdd/GaoHZW12: 
conf/sdm/SchubertWZK12: 
conf/kdd/ZimekGCS13: 
RayanaAkoglu14: full ensemble
}


Feature bagging~\cite{conf/kdd/LazarevicK05} is the earliest work formalizing an outlier ensemble. It uses the same base algorithm (i.e., LOF~\cite{Markus2000}) on different feature subsets and employs a rank based merging to create the final consensus. Feature bagging is better calibrated by~\cite{conf/icdm/GaoT06, conf/sdm/KriegelKSZ11} which convert the outlier scores to probability estimates and use score based merging. %In our work, we leverage both rank based and score based aggregation to find consensus. 
Different from those, 
\cite{conf/pakdd/GaoHZW12,RayanaAkoglu14,conf/sdm/SchubertWZK12,conf/dasfaa/VuAG10,conf/kdd/ZimekGCS13} utilize heterogeneous detectors (e.g., LOF~\cite{Markus2000}, LOCI \cite{DBLP:conf/icde/PapadimitriouKGF03}, k-distance, etc.). Specifically, \cite{conf/pakdd/GaoHZW12,RayanaAkoglu14} unify and combine results from all detectors, \cite{conf/dasfaa/VuAG10} uses accuracy on synthetically generated datasets to assign weights to the detectors, and \cite{conf/sdm/SchubertWZK12,conf/kdd/ZimekGCS13} select the most diverse set of results to combine.
All these methods are designed for outlier detection in clouds of points. 

% merits of our work



%%\noindent{\em Time Series Anomaly Mining.}
%%...
%%
%%\noindent{\em Dynamic Graph Mining.}
%%...
%Ensembles for unsupervised outlier detection is an emerging topic that has been neglected for a long time compared to ensembles for classification and clustering problems \cite{conf/mcs/Dietterich00,conf/wirn/ValentiniM02,books/crc/aggarwal13/GhoshA13}. This is because in unsupervised settings no ground truth is available to evaluate the merit of the ensemble over its components. 
%Moreover, unlike in clustering which falls under unsupervised learning, there exists no objective or fitness functions for outlier mining.
%Nevertheless, there have been several recent works on building outlier ensembles. In a recent position paper, Aggarwal~\cite{EnsembleCharu} provided a categorization of the existing outlier ensemble approaches based on corresponding algorithmic strategies. According to Aggarwal, there have been traces of the very idea of combining results from different models in many earlier works but none of them are explicitly named as ensemble approaches. 
%
%In particular, ensemble approach is effectively used in high-dimensional outlier detection~\cite{EnsembleCharu} where multiple subspaces of data are explored to detect outliers. The feature bagging approach~\cite{Lazarevic05featurebagging} is the earliest work formalizing an outlier ensemble in high dimensional feature space, as outlier behavior of data points are often described by a subset of the dimensions. This approach uses the same base algorithm (LOF~\cite{Markus2000}) on different feature subsets and provides a rank based merging to create the final consensus. Feature bagging is better calibrated by~\cite{Jing06MM, Zimek11Uni} which convert the outlier scores to probability estimates and use a score based merging. Our approach in contrast uses both rank based and score based aggregation to build the final ensemble.
%
%In addition to using the variants of the same algorithm as ensemble components, it is possible to use different algorithms to build a heterogeneous ensemble. In~\cite{Nguyen2010} Nguyen et al. use both LOF~\cite{Markus2000} and LOCI~\cite{Faloutsos2003} (density based outlier detectors) as components of their ensemble. While their approach is similar to ours, we build a heterogeneous ensemble for dynamic graphs in contrast to static clouds of points and capture the time evolving behavior of the data. Other existing outlier ensembles are also designed for clouds of multi-dimensional data points. 
%
%According to Zimek et al.~\cite{}, the two core ingredients of ensemble construction are accuracy and diversity. Considering event detection as an unsupervised problem nothing is known about the accuracy of individual event detectors. But the effect of diversity of the individual detectors on designing better ensembles has been studied extensively in ensemble clustering~\cite{}. They provide a greedy approach~\cite{} to select the diverse detectors to build the final ensemble to reduce redundancy. Our previous work on ensemble design~\cite{Rayana2014} reveals the fact that too much diversity among the base detectors hurts the final ensemble. Similarly, in data fusion where web data from different sources are combined to build a knowledge base too much noise in several individual sources hurts the knowledge base. Srivastava et al.~\cite{} provide a greedy approach to select the correlated data sources for data fusion to remove the erroneous data sources.  
%
%
%
%
%%To the best of our knowledge, ours is the first ensemble approach for event detection in time-evolving graph data. 
